Dual Online Stein Variational Inference for Control and Dynamics

Model predictive control (MPC) schemes have a proven track record for delivering aggressive and robust performance in many challenging control tasks, coping with nonlinear system dynamics, constraints, and observational noise. Despite their success, these methods often rely on simple control distributions, which can limit their performance in highly uncertain and complex environments. MPC frameworks must be able to accommodate changing distributions over system parameters, based on the most recent measurements. In this paper, we devise an implicit variational inference algorithm able to estimate distributions over model parameters and control inputs on-the-fly. The method incorporates Stein Variational gradient descent to approximate the target distributions as a collection of particles, and performs updates based on a Bayesian formulation. This enables the approximation of complex multi-modal posterior distributions, typically occurring in challenging and realistic robot navigation tasks. We demonstrate our approach on both simulated and real-world experiments requiring real-time execution in the face of dynamically changing environments.

==> snippets.tex <==
We can now modify \cref{eq:dsvmpc_joint_likelihood} to condition the probability
density of $\simParams$ to the observed data $\dataset$, namely:
\begin{equation} \label{eq:dsvmpc_exact_likelihood}
    p(\polParams, \simParams \given \optimality)
    \propto \int_\trajectorySpace p(\optimality \given \trajectory)
    p(\trajectory \given \polParams, \simParams) p(\polParams)
    p(\simParams \given \dataset)
    \diff\trajectory \,,
\end{equation}
where the dependence on $\dataset$ is denoted only on the posterior over dynamics
parameters $p(\simParams \given \dataset)$ for simplicity.
As an aside, one implication of \cref{eq:dsvmpc_exact_likelihood} is how
$\dataset$ is initialised, if bootstrapped with initial data collection or based
on a prior defined by domain knowledge.
In either case, we now need a way to update our posterior $p(\simParams
\given \dataset)$ in light of new observations.

One approach, shared by \cite{okada_variational_2019, ramos_bayessim:_2019, possasOnlineBayesSimCombined},
is to bootstrap our dataset and train an initial estimate of $\pDensity(\simParams
\given \dataset)$.
As discussed on \cref{sec:related_work}, each of these methods uses different
strategies are used to solve the inference
problem, however all share the same principle of updating the posterior density
in an \textit{episodic} setting.



% Since $\simParams$ parameterises a transition function $\simFunction$ usually 
% associated with spatial displacement, we postulate that a Normal distribution 
% centred around the newly observed $\state_\tIdx^r$ is a suitable metric for 
% the likelihood function.
% More formally we have:
% \begin{equation}
% \begin{split}
%     &= \int_\stateSpace \pDensity(\datapoint \given \state_\tIdx, \simParams)
%     \pDensity(
%     \state_\tIdx \given \state_{\tIdx - 1}^r, \control_{\tIdx - 1}^r, \simParams
%     ) \diff\state_\tIdx \\
%     &= \int_\stateSpace
%     \normal(\state_\tIdx \given \state_\tIdx^r, \sigma^2 \mat{I})
%     \simDensity(\state_\tIdx \given \state_{\tIdx - 1}^r, \control_{\tIdx - 1}^r)
%     \diff\state_\tIdx \,,
% \end{split}
% \end{equation}
% where $\pDensity(\datapoint \given \simParams)$ the variance $\sigma^2$ can be learned experimentally.


GENERAL IDEAS:
\begin{itemize}
    \item If fitting a Gaussian centred on the latest observed state, could the last SVMPC bandwidth be a good indication of the variance to use?
\end{itemize}
